HACK3D: Crowdsourcing the Assessment of Cybersecurity in Digital Manufacturing

Digital manufacturing (DM) cyber-physical system is vulnerable to both cyber and physical attacks. HACK3D is a series of crowdsourcing red-team-blue-team events hosted by the NYU Center for Cybersecurity to assess the strength of the security methods embedded in designs using DM. This study summarizes the lessons learned from the past three offerings of HACK3D, including ingenious ways in which skilled engineers can launch surprising attacks on DM designs not anticipated before. A key outcome is a taxonomy-guided creation of DM security benchmarks for use by the DM community.

==> experiments.tex <==
\section{Experimental Evaluation}\label{s:experiments}
In order to assess the impact of attacks on the physical properties of AM printed artifacts, and the effectiveness of standard testing methods, we use a standard ``dogbone'' tensile specimen as our case study. %
In the following paragraphs we present our experimental results for two attack vectors discussed in Section \ref{s:attacks}.


\subsection{Methodology and Experimental Setup}\label{ss:method}
The test specimens are printed and tested according to the ASTM E8 standard using the following AM flow: (i) design the specimen using SolidWorks 2014 CAD and CSG software, (ii) slice the design using Catalyst EX 4.4 software with the solid fill option and $0.01$ inch layer height, (iii) print using FDM technology\footnote{Different printers and materials are used for each attack}, and (iv) test all specimens (both attacks) under tensile loading conditions using an Instron 4467 test machine equipped with a $30$ kN load cell and a $1$ inch gauge length Instron extensometer for obtaining strain data. For the second attack vector, we performed non-destructive testing using an Physical Acoustics Ultrapac 1000 ultrasonic scanner, while we performed FEA simulations using Ansys 15.0 software.

\begin{figure}[t]
  \centering
  \subfloat[]{\label{f:exp_2} %
  	\includegraphics[width=1.6in]{imgs/media/image2.png}} 
  \subfloat[]{\label{f:exp_3} %
  	\includegraphics[width=1.6in]{imgs/media/image3.png}} \\ 
  	\vspace{-0.10in}
  \subfloat[]{\label{f:exp_4} %
  	\includegraphics[width=1.6in]{imgs/media/image4.png}}  
  \subfloat[]{\label{f:exp_5} %
  	\raisebox{0.30in}{\includegraphics[width=1.6in]{imgs/media/image5.png}}} 	%
 \caption{AM printed tensile specimens. First attack: (a) print orientation $45^\circ$ from the long axis; (b) print orientation parallel to the $x$ axis; (c) print direction parallel to the $z$ axis. Second attack: (d) print in the plane of the print bed with a cubic defect (edge length $150$ $\mu m$).} 
  \label{f:exp_2_5}
\end{figure}

\subsection{Modified Print Orientation (first attack)}\label{ss:orientation}
In this attack, we alter the direction of printing with respect to the movement of the extrusion head. The specimens are printed using Stratasys Dimension Elite FDM 3D printer and ``ABSplus'' filament and were subjected to tensile tests. Fig. \ref{f:exp_2}--\ref{f:exp_4} shows three printing directions with respect to the specimen geometry. Change in orientation could be inserted during slicing or by maliciously modifying the toolpath files.

\subsubsection{Strength Test Results}\label{sss:exp_strength1}
The experimental results from the tensile tests for the first attack are compiled in Fig. \ref{f:exp_6}, using five specimens in each orientation. In the interest of brevity and clarity we only included only one specimen in the graph). Table \ref{t:tensile} shows the test results. From the results, observe that except 
for the modulus of $z$-direction orientation, the standard deviation is
below $6\%$ for modulus and strength values of all specimens. Compared to
the $z$-direction orientation, the $x$ and $45^\circ$ specimens have 
$15\%$ and $4\%$ higher modulus, respectively. The strength 
values of $x$ and $45^\circ$ specimens are $22\%$ and $4\%$ higher, 
respectively, compared to the $z$-direction specimens. These results show 
that the $45^\circ$ printing orientation is the best.%
Thus, if the original  model is oriented at $45^\circ$ direction for printing, any attack in the 
printing direction for the same model can significantly lower the strength 
and modulus and make the part under perform compared to the design conditions.

Failure strain is another parameter of interest. Fig. \ref{f:exp_6}  
shows that the failure strain is significantly compromised when the
printing direction is changed. The $45^\circ$ orientation provides over 
$2.5\%$ strain before failure, while the other two orientations have less 
than $1.5\%$ strain. Reduction in failure strain can reduce the response time
available for intervention or repair and increases the possibility of
catastrophic failure.

\begin{figure}[t]
  \centering

  \subfloat[]{\label{f:exp_6} %
  	\includegraphics[width=1.6in]{imgs/media/image6.png}} 
  \subfloat[]{\label{f:exp_9} %
  	\includegraphics[width=1.6in]{imgs/media/image9.png}} 
  
  \caption{First attack: (a) Stress-strain curves for representative specimens fabricated in each orientation. Second Attack: (b) Stress-strain curves for tensile bars with defect embedded at the center, for $[15^\circ,15^\circ]$ and $90^\circ$ print orientations. %
  } 
  \label{f:exp_6_9}
\end{figure}


\begin{table}[t]
 \caption{Experimental results for elastic modulus and strength (first attack).}
 \label{t:tensile}
 \begin{center}
 \renewcommand{\arraystretch}{1.2} 
 \begin{tabular} {|c|c|c|}
 
 \hline
 
 \multirow{2}{*}{\parbox{0.7in}{\centering {\bf Printing Orientation}}} & 
 \multirow{2}{*}{\parbox{0.9in}{\centering {\bf Modulus (GPa)}}} &
 \multirow{2}{*}{\parbox{0.9in}{\centering {\bf Strength (MPa)}}} \\ 
 & & \\ \hline \hline
 
 {\bf x} & 
 $2.27 \pm 0.08$  &   
 $33.31 \pm 1.31$ 
 \\ \hline
 
 {\bf $45^\circ$} & 
 $2.02 \pm 0.05$ &   
 $25.48 \pm 1.6$ 
 \\ \hline
 
 {\bf z} & 
 $1.97 \pm 0.24$ &   
 $27.38 \pm 1.58$ 
 \\ \hline

 \end{tabular}
 \end{center}
 \end{table}


\subsection{Contaminant Insertion (second attack)}\label{ss:contaminant}
A specimen is printed with a small defect embedded at the center. The defect is created by printing a square section feature of a soft elastomer-like material. From a mechanical perspective, this defect simulates either a void inside the specimen or insertion of a foreign material. We printed the defective specimens in two different printing orientations (Fig. \ref{f:exp_8}), with respect to the print head movement, using a Stratasys Connex500 printer with ``Vero Clear'' as the main material and ``Tango Black Plus'' as the contaminant (shown in Fig. \ref{f:exp_5}). Specimens of both print orientations are subjected to tensile tests and ultrasonic evaluation using C-scan mode and a $5$ MHz frequency transducer with $1$~in focal distance and water coupling in the pulse-echo mode.

Besides physical testing, we conduct FEA simulations on the 3D models by %
assigning elastic modulus and Poisson's ratio of the material to be $2.2$ GPa
and $0.35$ respectively. We did a convergence study in order to
select the appropriate mesh size for all models and obtain results that
are mesh independent. We also obtained the convergence in displacement. The FEA study involves simulating an ``intact'' tensile specimen to generate baseline properties. For the malicious specimen, the defect is incorporated at the center and we observe its effect on the specimen
response for different defect sizes and locations along the thickness direction.

\subsubsection{Ultrasonic Test Results}\label{sss:exp_us2}
The 3D printed defective tensile test specimens are scanned using
ultrasonic C-scan to characterize their physical state before
tensile testing. The C-scan time of flight results are presented in
Fig. \ref{f:exp_7} for the two specimens. These specimens have a defect at the center. The surface texture due to the printing direction  can be resolved in these figures. The top image has layers printed along
x-direction but at $15^\circ$ angles from the $y$ and $z$ directions. Therefore, the longitudinal texture is identified in the top figure. The  specimens were printed at this angle so that the small size defect feature  can be printed with greater accuracy compared to the printing in $x$ or
$y$ direction. The bottom figure is printed in the perpendicular
direction, which also be identified. However, the defect cannot be
resolved due to the small size and presence of features related to
surface texture that mask the internal defect.

From the results, it appears that the direction of printing can be
identified from the C-scan test with sufficiently high frequency.
Identification of an internal defect depends on the defect size and
location and the presence of other features that may mask the
defect. The attenuation in \emph{viscoelastic polymers} is usually higher compared to \emph{thermosets} and metals,  leading to the use of lower test frequencies. Similar testing can be 
conducted in metallic specimens at $20$ MHz frequency, which will 
significantly increase the resolution in the C-scan results.


\begin{figure}[t]
  \centering
  \subfloat[]{\label{f:exp_7} %
  	\includegraphics[width=1.6in]{imgs/media/image7.png}}
  \subfloat[]{\label{f:exp_8} %
  	\includegraphics[width=1.6in]{imgs/media/image8.png}}

  
  \caption{Second attack: (a) Ultrasonic C-scan images of specimens with defect embedded at the center, for $[15^\circ,15^\circ]$ and $90^\circ$ print orientations. The scan represents time of flight results, while the color scale represents depth (all scales in inch units). %
  (b) Two specimen orientations with respect to the printing direction for specimens with embedded defect at the center. 
  } 
  \label{f:exp_7_8}
\end{figure}

\subsubsection{Strength Test Results}\label{sss:exp_strength2}

Testing the defective specimens for both print orientations (Fig. \ref{f:exp_7_8}), demonstrates correlation between strength and print direction; the orientation has a significant impact on the measured 
tensile properties of the specimens (Fig. \ref{f:exp_9}). The $15^\circ$ print-orientation specimens have strength of $37.6$ MPa, compared to 
$31.3$ MPa of the specimens printed
``in-plane''. Since both specimens have the same size defect, the presence
of defect is not a parameter in comparing their properties. The
transparent specimens allowed monitoring of the defect and the crack
initiation and propagation during testing. Due to the small size, the
defect did not appear to influence the deformation behavior of the
specimen and the fracture originated elsewhere.

Presence of such small defects may be undetected during tensile testing
because there is always some variation in the measured values for
the specimens of the same type (e.g., up to about $6\%$ variation is
observed for intact specimens). However, in scenarios where 3D printed
components are used under rigorous conditions, such as molding dies at
high temperature and pressure for millions of molding cycles, such
defects may become locations of \emph{stress concentration}\footnote{The stress concentration is defined as the ratio of the maximum stress from the simulation to the nominal stress for the cross section.} and grow over time.


\subsubsection{Finite Element Analysis Results}\label{sss:exp_fea2}

A discretized model of an intact tensile test specimen is shown in
Fig. \ref{f:exp_10}, where the specimen is constrained in the longitudinal
direction and a force of $1$ kN is applied at the other end. The specimens
are modeled as homogeneous and isotropic materials. The FEA simulation of the intact specimen (visualized in Fig. \ref{f:exp_11}), show that
that maximum \emph{von-Mises stress} obtained in this specimen geometry is 
$107.98$ MPa and the location of the maximum is in the shoulder region. 
On the other hand, the outer surfaces of two simulated models \emph{containing 
internal defects} are shown in Fig. \ref{f:exp_12}--\ref{f:exp_13}. 
Compared to the intact specimen results (Fig. \ref{f:exp_10}), 
the location of maximum stress is not observed at the shoulder of
the curvature in the defective models.

The FEA results for the specimens with embedded defects of various sizes
at the center are shown in Fig. \ref{f:exp_14}--\ref{f:exp_16}. In 
comparison, Fig. \ref{f:exp_17}--\ref{f:exp_19} demonstrate the equivalent stress when a same size defect is moved to a different location along the 
specimen thickness. Our simulation shows that the maximum stress occurs around the void, instead of the curvature shoulder as in the intact model. The values of maximum von-Mises stress for the specimens having defects of 
different sizes and at different locations are compiled in Table 
\ref{t:fea1}. The simulated stress for the intact model at the same location as 
the defect is $83$ MPa, which indicates a swift in the location of the maximum 
stress point from the shoulder (intact model) to the defect point (defective 
model). For all defective specimens, the 
maximum observed von-Mises stress is also higher than the value observed for 
the intact specimen (i.e. $107.98$ MPa). For both depth locations (i.e. center 
and midway to surface), the stress concentration increases with the size of the 
square cross section defect (Table \ref{t:fea2}).

\begin{table}[t]
 \caption{Maximum von-Mises stress from FEA of defective tensile specimens (second attack).}
 \label{t:fea1}
 \begin{center}
 \renewcommand{\arraystretch}{1.2} 
 \begin{tabular} {|c|c|c|}
 
 \hline
 
 \multirow{3}{*}{\parbox{0.9in}{\centering {\bf Defect Size}}} &
 \multicolumn{2}{c|} {\bf Maximum von-Mises Stress (MPa)} \\ \cline{2-3}
 &
 \multirow{2}{*}{\parbox{1.0in}{\centering {\bf At 1 mm Depth (Center)}}} &
 \multirow{2}{*}{\parbox{0.95in}{\centering {\bf At 0.5 mm Depth (Midway)}}} \\ 
 & & \\ 
 \hline \hline
 
 {\bf $150 \mu m$} & 
 $123.8$  &   
 $121.4$ 
 \\ \hline
 
 {\bf $250 \mu m$} & 
 $124.7$ &   
 $124.1$ 
 \\ \hline
 
 {\bf $500 \mu m$} & 
 $126.1$ &   
 $130.6$ 
 \\ \hline

 \end{tabular}
 \end{center}
 \end{table}

\begin{table}[t]
 \caption{Stress concentrations from FEA of defective specimens (second attack).}
 \label{t:fea2}
 \begin{center}
 \renewcommand{\arraystretch}{1.2} 
 \begin{tabular} {|c|c|c|}
 
 \hline
 
 \multirow{3}{*}{\parbox{0.9in}{\centering {\bf Defect Size}}} &
 \multicolumn{2}{c|} {\bf Stress Concentration} \\ \cline{2-3}
 &
 \multirow{2}{*}{\parbox{1.0in}{\centering {\bf At 1 mm Depth (Center)}}} &
 \multirow{2}{*}{\parbox{0.95in}{\centering {\bf At 0.5 mm Depth (Midway)}}} \\ 
 & & \\ 
 \hline \hline
 
 {\bf $150 \mu m$} & 
 $1.486$  &   
 $1.457$ 
 \\ \hline
 
 {\bf $250 \mu m$} & 
 $1.497$ &   
 $1.490$ 
 \\ \hline
 
 {\bf $500 \mu m$} & 
 $1.514$ &   
 $1.568$ 
 \\ \hline

 \end{tabular}
 \end{center}
 \end{table}

\begin{figure}[t]
  \centering

  \subfloat[]{\label{f:exp_10} %
  	\raisebox{0.30in}{\includegraphics[width=1.6in]{imgs/media/image10.png}}}
  \subfloat[]{\label{f:exp_11} %
  	\includegraphics[width=1.6in]{imgs/media/image11.png}} 
  
  \caption{Second attack: (a) A meshed model and boundary conditions used in FEA. (b) FEA simulation of tension test on (isotropic) 3D printed specimens with no defect. The maximum equivalent stress is on the shoulder region, and all of the tested specimens fail in this region. The average stress in the reduced section is $83$ MPa at the simulated load of $1$ kN. This stress value is used as the nominal stress for finding the concentrations caused by the presence of a defect.} 
  \label{f:exp_10_11}
\end{figure}


\begin{figure}[t]
  \centering

  \subfloat[]{\label{f:exp_12} %
  	\includegraphics[width=1.6in]{imgs/media/image12.png}} 
  \subfloat[]{\label{f:exp_13} %
  	\includegraphics[width=1.6in]{imgs/media/image13.png}} 
  
  \caption{Second attack: Top views of the FEA results on defective specimens. The internal defects in (a) and (b) are cross-referenced with in Fig. \ref{f:exp_14} and \ref{f:exp_19}, respectively.} 
  \label{f:exp_12_13}
\end{figure}


\begin{figure}[t]
  \centering

  \subfloat[]{\label{f:exp_14} %
  	\includegraphics[width=1.6in]{imgs/media/image14.png}} 
  \subfloat[]{\label{f:exp_15} %
  	\includegraphics[width=1.6in]{imgs/media/image15.png}} \\
  	\vspace{-0.10in}
  \subfloat[]{\label{f:exp_16} %
  	\includegraphics[width=1.6in]{imgs/media/image16.png}} 
  \subfloat[]{\label{f:exp_17} %
  	\includegraphics[width=1.6in]{imgs/media/image17.png}} \\
  	\vspace{-0.10in}
  \subfloat[]{\label{f:exp_18} %
  	\includegraphics[width=1.6in]{imgs/media/image18.png}}
  \subfloat[]{\label{f:exp_19} %
  	\includegraphics[width=1.6in]{imgs/media/image19.png}} 
  
  \caption{Second attack: FEA simulations of embedded defects in tensile bars. The stress distribution away from the defect is identical to that shown in Fig. \ref{f:exp_11} for the non-defective specimen. (a)--(c) Stress distribution for centrally placed defect size from $150-500 \mu m$. (d)--(f) Stress distribution a defect placed midway between the center and the surface (same size ranges).} 
  \label{f:exp_14_19}
\end{figure}


\subsection{Analysis of Experimental Results}\label{ss:exp_summary}

Our results demonstrate that the FDM print direction has a strong impact
on the measured mechanical properties of the specimen. The expected
strength and modulus are affected by the polymer layering orientation with
respect to the specimen axis. Furthermore, the results indicate that contamination with a different material or voids modifies the stress concentration in the artifact.

In practice, attackers may implement the first attack by changing in coordinate system of the printer itself compared to the drawing software. In certain cases this change may be as simple as issuing a few G-code commands. In other cases, attackers may operate the slicing software and reorient the artifact before layers and toolpaths are generated. As our results indicate, detection of the first attack is possible though ultrasonic testing and destructive tensile tests.

Regarding the second attack, attackers can introduce directly at the .STL file or even in the G-code. On the other hand, if the attack is introduced at the design step, FEA simulations would most probably demonstrate changes in maximum stress and stress concentrations allowing detection. Our results indicate that this attack maybe remain undetected by destructive tensile tests (due to adequately large standard deviation in specification), as well as ultrasonic tests (due to the small defect size). Nevertheless, due to stress concentration and repeated loading, the defect would grow over time and cause premature failure of the component.









